Rethinking Few-Shot Object Detection on a Multi-Domain Benchmark

Most existing works on few-shot object detection (FSOD) focus on a setting where both pre-training and few-shot learning datasets are from a similar domain. However, few-shot algorithms are important in multiple domains; hence evaluation needs to reflect the broad applications. We propose a Multi-dOmain Few-Shot Object Detection (MoFSOD) benchmark consisting of 10 datasets from a wide range of domains to evaluate FSOD algorithms. We comprehensively analyze the impacts of freezing layers, different architectures, and different pre-training datasets on FSOD performance. Our empirical results show several key factors that have not been explored in previous works: 1) contrary to previous belief, on a multi-domain benchmark, fine-tuning (FT) is a strong baseline for FSOD, performing on par or better than the state-of-the-art (SOTA) algorithms; 2) utilizing FT as the baseline allows us to explore multiple architectures, and we found them to have a significant impact on down-stream few-shot tasks, even with similar pre-training performances; 3) by decoupling pre-training and few-shot learning, MoFSOD allows us to explore the impact of different pre-training datasets, and the right choice can boost the performance of the down-stream tasks significantly. Based on these findings, we list possible avenues of investigation for improving FSOD performance and propose two simple modifications to existing algorithms that lead to SOTA performance on the MoFSOD benchmark. The code is available at https://github.com/amazon-research/few-shot-object-detection-benchmark.

==> table_32.tex <==
\begin{sidewaystable*}[t]
\def\smidrulea{\cmidrule(rl){2-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(rl){9-11}\cmidrule(rl){12-12}\cmidrule(rl){13-13}\cmidrule(rl){14-15}\cmidrule(rl){16-17}\cmidrule(rl){18-18}}
\def\smidruleb{\cmidrule(rl){2-3}\cmidrule(rl){4-5}\cmidrule(rl){6-7}\cmidrule(rl){8-9}\cmidrule(rl){10-10}\cmidrule(rl){11-11}\cmidrule(rl){12-15}\cmidrule(rl){16-16}}
\def\smidrulec{\cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}\cmidrule(rl){6-6}\cmidrule(rl){7-7}\cmidrule(rl){8-8}\cmidrule(rl){9-9}\cmidrule(rl){10-10}\cmidrule(rl){11-11}\cmidrule(rl){12-12}\cmidrule(rl){13-13}\cmidrule(rl){14-14}\cmidrule(rl){15-15}\cmidrule(rl){16-16}\cmidrule(rl){17-17}\cmidrule(rl){18-18}}
\centering
%\setlength{\tabcolsep}{1mm}
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{cccccccccccccccccc}
\toprule
\multirowcell{2}{1-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
& CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
67.7 \scriptsize{$\pm$ 3.5} & 5.8 \scriptsize{$\pm$ 1.0} & 7.1 \scriptsize{$\pm$ 0.4} & 32.8 \scriptsize{$\pm$ 4.3} & 29.2 \scriptsize{$\pm$ 8.4} & 19.0 \scriptsize{$\pm$ 2.4} & 53.7 \scriptsize{$\pm$ 19.7} & 31.2 \scriptsize{$\pm$ 2.6} & 14.8 \scriptsize{$\pm$ 3.9} & \textbf{34.7} \scriptsize{$\pm$ 5.9} & 32.6 \scriptsize{$\pm$ 7.0} & 0.5 \scriptsize{$\pm$ 0.5} & 4.9 \scriptsize{$\pm$ 0.5} & 7.0 \scriptsize{$\pm$ 1.0} & 65.1 \scriptsize{$\pm$ 5.5} & 18.8 \scriptsize{$\pm$ 2.5} & 7.1 \scriptsize{$\pm$ 6.8} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
68.0 \scriptsize{$\pm$ 3.2} & 5.9 \scriptsize{$\pm$ 1.3} & 7.4 \scriptsize{$\pm$ 0.5} & 32.3 \scriptsize{$\pm$ 4.4} & 31.4 \scriptsize{$\pm$ 7.4} & 19.4 \scriptsize{$\pm$ 2.4} & 55.7 \scriptsize{$\pm$ 19.7} & 31.0 \scriptsize{$\pm$ 2.0} & 15.9 \scriptsize{$\pm$ 4.0} & 34.6 \scriptsize{$\pm$ 5.4} & 33.9 \scriptsize{$\pm$ 6.7} & 0.5 \scriptsize{$\pm$ 0.5} & 4.8 \scriptsize{$\pm$ 0.6} & 6.9 \scriptsize{$\pm$ 1.2} & 65.0 \scriptsize{$\pm$ 5.5} & 17.3 \scriptsize{$\pm$ 2.0} & 7.5 \scriptsize{$\pm$ 6.7} \cr
FSCE-base~\cite{sun2021fsce} &
71.3 \scriptsize{$\pm$ 6.2} & 11.2 \scriptsize{$\pm$ 2.2} & 7.6 \scriptsize{$\pm$ 0.8} & 35.7 \scriptsize{$\pm$ 6.0} & 32.2 \scriptsize{$\pm$ 13.9} & 20.8 \scriptsize{$\pm$ 2.7} & 57.9 \scriptsize{$\pm$ 10.7} & 28.5 \scriptsize{$\pm$ 2.7} & 15.0 \scriptsize{$\pm$ 3.9} & 34.0 \scriptsize{$\pm$ 4.5} & 37.2 \scriptsize{$\pm$ 8.9} & 12.4 \scriptsize{$\pm$ 8.3} & 7.2 \scriptsize{$\pm$ 1.3} & 14.0 \scriptsize{$\pm$ 1.3} & 75.2 \scriptsize{$\pm$ 7.9} & 33.7 \scriptsize{$\pm$ 4.6} & 34.6 \scriptsize{$\pm$ 20.3} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
72.2 \scriptsize{$\pm$ 5.6} & 11.9 \scriptsize{$\pm$ 2.2} & 7.6 \scriptsize{$\pm$ 0.9} & 36.0 \scriptsize{$\pm$ 5.5} & 31.8 \scriptsize{$\pm$ 14.1} & 20.5 \scriptsize{$\pm$ 2.9} & 57.9 \scriptsize{$\pm$ 12.5} & 30.4 \scriptsize{$\pm$ 2.6} & 14.9 \scriptsize{$\pm$ 3.8} & 34.3 \scriptsize{$\pm$ 5.2} & \textbf{37.8} \scriptsize{$\pm$ 8.7} & \textbf{13.1} \scriptsize{$\pm$ 8.1} & 7.5 \scriptsize{$\pm$ 1.3} & \textbf{14.6} \scriptsize{$\pm$ 1.4} & \textbf{77.3} \scriptsize{$\pm$ 7.9} & 36.3 \scriptsize{$\pm$ 5.5} & 35.9 \scriptsize{$\pm$ 21.3} \cr
DeFRCN~\cite{qiao2021defrcn} &
71.5 \scriptsize{$\pm$ 8.9} & 12.9 \scriptsize{$\pm$ 2.6} & 6.1 \scriptsize{$\pm$ 0.8} & \textbf{45.1} \scriptsize{$\pm$ 5.8} & 30.8 \scriptsize{$\pm$ 9.0} & \textbf{27.8} \scriptsize{$\pm$ 3.0} & 50.5 \scriptsize{$\pm$ 10.1} & 25.5 \scriptsize{$\pm$ 2.4} & 17.4 \scriptsize{$\pm$ 4.5} & 25.6 \scriptsize{$\pm$ 3.1} & 34.9 \scriptsize{$\pm$ 6.0} & 8.9 \scriptsize{$\pm$ 6.4} & 8.6 \scriptsize{$\pm$ 1.6} & 13.7 \scriptsize{$\pm$ 1.2} & 76.4 \scriptsize{$\pm$ 6.4} & 42.6 \scriptsize{$\pm$ 6.4} & \textbf{36.1} \scriptsize{$\pm$ 21.3} \cr
\rowcolor{Gray} FT &
\textbf{76.0} \scriptsize{$\pm$ 3.0} & \textbf{13.8} \scriptsize{$\pm$ 2.5} & \textbf{7.7} \scriptsize{$\pm$ 0.7} & 33.8 \scriptsize{$\pm$ 8.1} & \textbf{33.0} \scriptsize{$\pm$ 7.6} & 18.4 \scriptsize{$\pm$ 1.6} & \textbf{60.5} \scriptsize{$\pm$ 5.3} & \textbf{34.9} \scriptsize{$\pm$ 4.6} & \textbf{21.4} \scriptsize{$\pm$ 5.3} & 32.2 \scriptsize{$\pm$ 4.1} & 35.4 \scriptsize{$\pm$ 8.5} & 11.7 \scriptsize{$\pm$ 7.6} & \textbf{9.7} \scriptsize{$\pm$ 2.2} & 12.9 \scriptsize{$\pm$ 1.1} & 71.2 \scriptsize{$\pm$ 8.1} & \textbf{43.0} \scriptsize{$\pm$ 6.6} & 33.0 \scriptsize{$\pm$ 17.2} \cr
\midrule
\multirowcell{2}{1-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
& LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
12.5 \scriptsize{$\pm$ 3.7} & 2.7 \scriptsize{$\pm$ 1.1} & 1.1 \scriptsize{$\pm$ 0.5} & 0.2 \scriptsize{$\pm$ 0.4} & 26.9 \scriptsize{$\pm$ 2.4} & 51.6 \scriptsize{$\pm$ 5.2} & 3.0 \scriptsize{$\pm$ 0.9} & 2.5 \scriptsize{$\pm$ 1.3} & 5.9 \scriptsize{$\pm$ 4.6} & 0.1 \scriptsize{$\pm$ 0.1} & 36.3 \scriptsize{$\pm$ 3.4} & \textbf{43.2} \scriptsize{$\pm$ 4.0} & 28.9 \scriptsize{$\pm$ 4.9} & 7.2 \scriptsize{$\pm$ 1.5} & 5.3 \scriptsize{$\pm$ 1.1} & 20.6 \scriptsize{$\pm$ 3.7} & 4.7 \scriptsize{$\pm$ 0.5} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
10.2 \scriptsize{$\pm$ 3.3} & 2.2 \scriptsize{$\pm$ 0.9} & 1.1 \scriptsize{$\pm$ 0.5} & 0.1 \scriptsize{$\pm$ 0.3} & 27.8 \scriptsize{$\pm$ 2.4} & \textbf{53.8} \scriptsize{$\pm$ 4.2} & 3.2 \scriptsize{$\pm$ 1.1} & 2.6 \scriptsize{$\pm$ 1.5} & 6.4 \scriptsize{$\pm$ 4.9} & 0.2 \scriptsize{$\pm$ 0.3} & \textbf{36.8} \scriptsize{$\pm$ 3.4} & 43.1 \scriptsize{$\pm$ 6.1} & 29.5 \scriptsize{$\pm$ 4.7} & 6.2 \scriptsize{$\pm$ 1.8} & 5.5 \scriptsize{$\pm$ 1.3} & 20.8 \scriptsize{$\pm$ 3.6} & 4.3 \scriptsize{$\pm$ 0.4} \cr
FSCE-base~\cite{sun2021fsce} &
21.8 \scriptsize{$\pm$ 5.2} & 7.5 \scriptsize{$\pm$ 1.3} & 2.3 \scriptsize{$\pm$ 0.6} & 0.1 \scriptsize{$\pm$ 0.3} & 43.6 \scriptsize{$\pm$ 5.0} & 52.3 \scriptsize{$\pm$ 3.2} & 5.1 \scriptsize{$\pm$ 1.1} & 4.5 \scriptsize{$\pm$ 2.7} & 9.0 \scriptsize{$\pm$ 5.7} & 0.9 \scriptsize{$\pm$ 0.6} & 30.0 \scriptsize{$\pm$ 1.7} & 40.6 \scriptsize{$\pm$ 6.4} & 32.0 \scriptsize{$\pm$ 5.0} & \textbf{17.2} \scriptsize{$\pm$ 2.5} & 12.6 \scriptsize{$\pm$ 1.5} & 25.3 \scriptsize{$\pm$ 4.2} & 3.3 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
23.5 \scriptsize{$\pm$ 5.7} & 8.4 \scriptsize{$\pm$ 1.6} & 2.3 \scriptsize{$\pm$ 0.6} & 0.2 \scriptsize{$\pm$ 0.2} & \textbf{44.0} \scriptsize{$\pm$ 4.7} & 51.8 \scriptsize{$\pm$ 3.6} & 5.3 \scriptsize{$\pm$ 1.3} & 4.3 \scriptsize{$\pm$ 2.7} & 10.4 \scriptsize{$\pm$ 6.6} & 1.2 \scriptsize{$\pm$ 0.6} & 30.4 \scriptsize{$\pm$ 1.7} & 40.3 \scriptsize{$\pm$ 5.9} & \textbf{34.5} \scriptsize{$\pm$ 5.0} & 16.6 \scriptsize{$\pm$ 2.9} & 13.4 \scriptsize{$\pm$ 1.6} & 25.8 \scriptsize{$\pm$ 4.4} & 2.8 \scriptsize{$\pm$ 0.4} \cr
DeFRCN~\cite{qiao2021defrcn} &
\textbf{27.6} \scriptsize{$\pm$ 5.3} & 8.8 \scriptsize{$\pm$ 1.8} & 2.7 \scriptsize{$\pm$ 0.5} & 0.0 \scriptsize{$\pm$ 0.0} & 39.5 \scriptsize{$\pm$ 4.1} & 49.5 \scriptsize{$\pm$ 4.5} & \textbf{10.5} \scriptsize{$\pm$ 3.3} & \textbf{8.1} \scriptsize{$\pm$ 5.2} & \textbf{20.9} \scriptsize{$\pm$ 7.4} & 0.3 \scriptsize{$\pm$ 0.2} & 28.7 \scriptsize{$\pm$ 2.5} & 38.3 \scriptsize{$\pm$ 5.0} & 24.4 \scriptsize{$\pm$ 4.6} & 7.5 \scriptsize{$\pm$ 1.4} & 13.2 \scriptsize{$\pm$ 1.9} & 25.4 \scriptsize{$\pm$ 4.0} & 3.3 \scriptsize{$\pm$ 0.5} \cr
\rowcolor{Gray} FT &
23.2 \scriptsize{$\pm$ 4.5} & \textbf{9.7} \scriptsize{$\pm$ 1.3} & \textbf{3.2} \scriptsize{$\pm$ 0.9} & \textbf{0.5} \scriptsize{$\pm$ 0.3} & 43.7 \scriptsize{$\pm$ 4.4} & 51.1 \scriptsize{$\pm$ 6.8} & 8.1 \scriptsize{$\pm$ 2.8} & 6.9 \scriptsize{$\pm$ 3.7} & 15.1 \scriptsize{$\pm$ 6.4} & \textbf{1.4} \scriptsize{$\pm$ 1.2} & 29.9 \scriptsize{$\pm$ 3.1} & 38.6 \scriptsize{$\pm$ 5.4} & 27.2 \scriptsize{$\pm$ 5.1} & 15.2 \scriptsize{$\pm$ 2.1} & \textbf{16.0} \scriptsize{$\pm$ 2.5} & \textbf{26.2} \scriptsize{$\pm$ 3.3} & \textbf{2.7} \scriptsize{$\pm$ 0.4} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{cccccccccccccccccc}
\toprule
\multirowcell{2}{3-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
& CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
72.4 \scriptsize{$\pm$ 0.9} & 8.9 \scriptsize{$\pm$ 1.1} & 8.8 \scriptsize{$\pm$ 0.4} & 44.6 \scriptsize{$\pm$ 4.2} & 39.4 \scriptsize{$\pm$ 5.6} & 26.6 \scriptsize{$\pm$ 1.7} & 70.0 \scriptsize{$\pm$ 4.4} & 37.8 \scriptsize{$\pm$ 2.2} & 18.5 \scriptsize{$\pm$ 4.0} & 37.9 \scriptsize{$\pm$ 5.5} & 39.1 \scriptsize{$\pm$ 3.6} & 1.0 \scriptsize{$\pm$ 0.5} & 7.4 \scriptsize{$\pm$ 0.9} & 8.5 \scriptsize{$\pm$ 1.2} & 74.0 \scriptsize{$\pm$ 2.6} & 30.5 \scriptsize{$\pm$ 6.0} & 18.7 \scriptsize{$\pm$ 8.5} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
72.3 \scriptsize{$\pm$ 1.0} & 8.8 \scriptsize{$\pm$ 1.1} & 9.1 \scriptsize{$\pm$ 0.4} & 43.9 \scriptsize{$\pm$ 3.4} & 40.5 \scriptsize{$\pm$ 5.3} & 26.1 \scriptsize{$\pm$ 1.5} & \textbf{70.9} \scriptsize{$\pm$ 3.9} & 37.8 \scriptsize{$\pm$ 1.7} & \textbf{19.0} \scriptsize{$\pm$ 3.7} & \textbf{38.0} \scriptsize{$\pm$ 5.7} & 39.7 \scriptsize{$\pm$ 3.3} & 1.0 \scriptsize{$\pm$ 0.5} & 7.4 \scriptsize{$\pm$ 0.9} & 8.1 \scriptsize{$\pm$ 0.9} & 74.6 \scriptsize{$\pm$ 2.7} & 27.2 \scriptsize{$\pm$ 5.2} & 18.8 \scriptsize{$\pm$ 9.1} \cr
FSCE-base~\cite{sun2021fsce} &
\textbf{79.2} \scriptsize{$\pm$ 1.2} & 19.1 \scriptsize{$\pm$ 2.9} & 10.9 \scriptsize{$\pm$ 0.7} & 50.7 \scriptsize{$\pm$ 5.7} & 45.0 \scriptsize{$\pm$ 9.6} & 33.5 \scriptsize{$\pm$ 1.8} & 69.5 \scriptsize{$\pm$ 2.5} & 37.8 \scriptsize{$\pm$ 2.5} & 17.2 \scriptsize{$\pm$ 3.6} & 35.4 \scriptsize{$\pm$ 5.2} & 44.9 \scriptsize{$\pm$ 3.9} & 28.0 \scriptsize{$\pm$ 5.9} & 14.9 \scriptsize{$\pm$ 1.0} & 19.5 \scriptsize{$\pm$ 1.0} & 87.2 \scriptsize{$\pm$ 3.0} & 54.0 \scriptsize{$\pm$ 7.0} & 49.9 \scriptsize{$\pm$ 22.4} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
79.0 \scriptsize{$\pm$ 1.1} & 19.6 \scriptsize{$\pm$ 2.9} & 11.0 \scriptsize{$\pm$ 0.8} & 51.0 \scriptsize{$\pm$ 5.3} & \textbf{45.2} \scriptsize{$\pm$ 9.8} & 33.7 \scriptsize{$\pm$ 2.3} & 68.0 \scriptsize{$\pm$ 3.0} & 39.1 \scriptsize{$\pm$ 2.5} & 17.3 \scriptsize{$\pm$ 4.1} & 35.9 \scriptsize{$\pm$ 5.6} & \textbf{45.0} \scriptsize{$\pm$ 3.8} & \textbf{29.1} \scriptsize{$\pm$ 5.7} & 15.1 \scriptsize{$\pm$ 1.2} & \textbf{19.8} \scriptsize{$\pm$ 0.8} & \textbf{88.5} \scriptsize{$\pm$ 3.0} & 57.7 \scriptsize{$\pm$ 7.3} & \textbf{55.3} \scriptsize{$\pm$ 21.3} \cr
DeFRCN~\cite{qiao2021defrcn} &
79.0 \scriptsize{$\pm$ 1.5} & 19.1 \scriptsize{$\pm$ 2.0} & 8.6 \scriptsize{$\pm$ 0.6} & \textbf{59.0} \scriptsize{$\pm$ 4.7} & 41.8 \scriptsize{$\pm$ 6.6} & \textbf{37.8} \scriptsize{$\pm$ 2.5} & 64.3 \scriptsize{$\pm$ 2.6} & 33.8 \scriptsize{$\pm$ 2.9} & 17.6 \scriptsize{$\pm$ 4.8} & 26.6 \scriptsize{$\pm$ 6.0} & 41.8 \scriptsize{$\pm$ 3.2} & 18.0 \scriptsize{$\pm$ 6.7} & 14.8 \scriptsize{$\pm$ 1.5} & 18.0 \scriptsize{$\pm$ 1.3} & 87.2 \scriptsize{$\pm$ 1.9} & 62.1 \scriptsize{$\pm$ 5.3} & 50.4 \scriptsize{$\pm$ 16.1} \cr
\rowcolor{Gray} FT &
78.9 \scriptsize{$\pm$ 0.6} & \textbf{22.0} \scriptsize{$\pm$ 2.6} & \textbf{11.4} \scriptsize{$\pm$ 0.7} & 52.4 \scriptsize{$\pm$ 4.3} & 43.6 \scriptsize{$\pm$ 9.8} & 30.6 \scriptsize{$\pm$ 1.8} & 67.5 \scriptsize{$\pm$ 3.5} & \textbf{44.6} \scriptsize{$\pm$ 3.9} & 19.0 \scriptsize{$\pm$ 4.5} & 32.7 \scriptsize{$\pm$ 3.9} & 43.5 \scriptsize{$\pm$ 3.1} & 26.3 \scriptsize{$\pm$ 4.9} & \textbf{16.7} \scriptsize{$\pm$ 1.6} & 18.9 \scriptsize{$\pm$ 1.1} & 86.7 \scriptsize{$\pm$ 2.8} & \textbf{64.7} \scriptsize{$\pm$ 7.2} & 53.1 \scriptsize{$\pm$ 17.1} \cr
\midrule
\multirowcell{2}{3-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
& LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
15.0 \scriptsize{$\pm$ 3.5} & 4.9 \scriptsize{$\pm$ 1.6} & 2.3 \scriptsize{$\pm$ 0.7} & 0.1 \scriptsize{$\pm$ 0.1} & 30.1 \scriptsize{$\pm$ 1.4} & 58.7 \scriptsize{$\pm$ 3.4} & 5.8 \scriptsize{$\pm$ 1.1} & 5.5 \scriptsize{$\pm$ 1.7} & 13.2 \scriptsize{$\pm$ 4.5} & 0.2 \scriptsize{$\pm$ 0.1} & 42.2 \scriptsize{$\pm$ 2.8} & 46.2 \scriptsize{$\pm$ 4.3} & 36.0 \scriptsize{$\pm$ 3.1} & 7.2 \scriptsize{$\pm$ 1.5} & 8.0 \scriptsize{$\pm$ 1.1} & 25.6 \scriptsize{$\pm$ 2.0} & 4.8 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
12.0 \scriptsize{$\pm$ 3.1} & 3.7 \scriptsize{$\pm$ 1.3} & 2.3 \scriptsize{$\pm$ 0.7} & 0.2 \scriptsize{$\pm$ 0.3} & 30.8 \scriptsize{$\pm$ 1.4} & \textbf{59.6} \scriptsize{$\pm$ 2.3} & 5.8 \scriptsize{$\pm$ 1.1} & 5.6 \scriptsize{$\pm$ 1.8} & 14.2 \scriptsize{$\pm$ 4.5} & 0.3 \scriptsize{$\pm$ 0.3} & \textbf{43.1} \scriptsize{$\pm$ 2.7} & \textbf{46.6} \scriptsize{$\pm$ 3.7} & 36.8 \scriptsize{$\pm$ 4.2} & 6.0 \scriptsize{$\pm$ 1.2} & 7.8 \scriptsize{$\pm$ 1.1} & 25.6 \scriptsize{$\pm$ 2.0} & 4.5 \scriptsize{$\pm$ 0.4} \cr
FSCE-base~\cite{sun2021fsce} &
36.7 \scriptsize{$\pm$ 5.3} & 15.2 \scriptsize{$\pm$ 1.8} & 4.7 \scriptsize{$\pm$ 1.2} & 0.4 \scriptsize{$\pm$ 0.4} & \textbf{49.3} \scriptsize{$\pm$ 2.7} & 55.5 \scriptsize{$\pm$ 2.2} & 10.3 \scriptsize{$\pm$ 1.7} & 9.5 \scriptsize{$\pm$ 3.5} & 21.3 \scriptsize{$\pm$ 5.4} & 2.6 \scriptsize{$\pm$ 1.3} & 35.9 \scriptsize{$\pm$ 3.4} & 44.7 \scriptsize{$\pm$ 4.4} & 45.9 \scriptsize{$\pm$ 4.4} & \textbf{26.3} \scriptsize{$\pm$ 3.5} & 21.0 \scriptsize{$\pm$ 2.7} & 33.6 \scriptsize{$\pm$ 3.9} & 3.0 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
36.4 \scriptsize{$\pm$ 5.2} & 16.4 \scriptsize{$\pm$ 1.4} & 4.8 \scriptsize{$\pm$ 1.1} & 0.3 \scriptsize{$\pm$ 0.3} & 48.8 \scriptsize{$\pm$ 3.0} & 55.2 \scriptsize{$\pm$ 1.7} & 10.8 \scriptsize{$\pm$ 1.8} & 10.2 \scriptsize{$\pm$ 3.6} & 21.9 \scriptsize{$\pm$ 5.3} & 3.0 \scriptsize{$\pm$ 1.5} & 35.1 \scriptsize{$\pm$ 3.0} & 44.8 \scriptsize{$\pm$ 4.6} & \textbf{48.3} \scriptsize{$\pm$ 4.4} & 22.3 \scriptsize{$\pm$ 2.6} & 21.8 \scriptsize{$\pm$ 3.4} & 34.1 \scriptsize{$\pm$ 3.7} & 2.7 \scriptsize{$\pm$ 0.3} \cr
DeFRCN~\cite{qiao2021defrcn} &
40.0 \scriptsize{$\pm$ 3.8} & 16.5 \scriptsize{$\pm$ 2.6} & 4.5 \scriptsize{$\pm$ 0.9} & 0.2 \scriptsize{$\pm$ 0.4} & 44.2 \scriptsize{$\pm$ 2.9} & 55.4 \scriptsize{$\pm$ 1.3} & \textbf{17.0} \scriptsize{$\pm$ 1.6} & \textbf{15.2} \scriptsize{$\pm$ 5.9} & 39.4 \scriptsize{$\pm$ 9.6} & 1.0 \scriptsize{$\pm$ 0.6} & 34.2 \scriptsize{$\pm$ 3.2} & 42.2 \scriptsize{$\pm$ 4.6} & 36.5 \scriptsize{$\pm$ 5.4} & 6.6 \scriptsize{$\pm$ 1.2} & 20.9 \scriptsize{$\pm$ 3.5} & 32.9 \scriptsize{$\pm$ 3.1} & 3.5 \scriptsize{$\pm$ 0.5} \cr
\rowcolor{Gray} FT &
\textbf{40.8} \scriptsize{$\pm$ 4.9} & \textbf{18.4} \scriptsize{$\pm$ 2.5} & \textbf{5.8} \scriptsize{$\pm$ 1.2} & \textbf{1.0} \scriptsize{$\pm$ 0.4} & 47.7 \scriptsize{$\pm$ 2.4} & 54.9 \scriptsize{$\pm$ 2.4} & 15.5 \scriptsize{$\pm$ 1.8} & 14.7 \scriptsize{$\pm$ 6.0} & \textbf{43.2} \scriptsize{$\pm$ 13.2} & \textbf{4.2} \scriptsize{$\pm$ 2.4} & 35.0 \scriptsize{$\pm$ 4.3} & 40.9 \scriptsize{$\pm$ 3.6} & 42.3 \scriptsize{$\pm$ 4.3} & 23.5 \scriptsize{$\pm$ 2.5} & \textbf{24.6} \scriptsize{$\pm$ 3.1} & \textbf{35.2} \scriptsize{$\pm$ 3.5} & \textbf{2.5} \scriptsize{$\pm$ 0.4} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{cccccccccccccccccc}
\toprule
\multirowcell{2}{5-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
& CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
72.5 \scriptsize{$\pm$ 0.8} & 10.7 \scriptsize{$\pm$ 1.2} & 9.7 \scriptsize{$\pm$ 0.5} & 50.6 \scriptsize{$\pm$ 1.9} & 43.0 \scriptsize{$\pm$ 2.1} & 31.0 \scriptsize{$\pm$ 2.2} & 71.8 \scriptsize{$\pm$ 2.8} & 42.5 \scriptsize{$\pm$ 2.4} & 18.6 \scriptsize{$\pm$ 2.7} & \textbf{40.9} \scriptsize{$\pm$ 5.1} & 40.0 \scriptsize{$\pm$ 2.0} & 1.3 \scriptsize{$\pm$ 0.5} & 8.7 \scriptsize{$\pm$ 1.2} & 8.6 \scriptsize{$\pm$ 0.9} & 76.3 \scriptsize{$\pm$ 1.8} & 36.9 \scriptsize{$\pm$ 4.3} & 27.5 \scriptsize{$\pm$ 7.3} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
72.3 \scriptsize{$\pm$ 0.7} & 10.8 \scriptsize{$\pm$ 1.1} & 9.8 \scriptsize{$\pm$ 0.4} & 49.0 \scriptsize{$\pm$ 2.2} & 44.0 \scriptsize{$\pm$ 2.1} & 30.1 \scriptsize{$\pm$ 2.3} & \textbf{72.5} \scriptsize{$\pm$ 2.6} & 42.1 \scriptsize{$\pm$ 2.7} & 19.2 \scriptsize{$\pm$ 3.0} & 40.3 \scriptsize{$\pm$ 4.9} & 40.4 \scriptsize{$\pm$ 2.2} & 1.4 \scriptsize{$\pm$ 0.5} & 8.6 \scriptsize{$\pm$ 1.0} & 8.0 \scriptsize{$\pm$ 0.7} & 76.8 \scriptsize{$\pm$ 1.7} & 33.5 \scriptsize{$\pm$ 4.2} & 27.8 \scriptsize{$\pm$ 7.4} \cr
FSCE-base~\cite{sun2021fsce} &
79.2 \scriptsize{$\pm$ 1.1} & 25.8 \scriptsize{$\pm$ 2.8} & 12.5 \scriptsize{$\pm$ 0.7} & 59.7 \scriptsize{$\pm$ 2.2} & 50.1 \scriptsize{$\pm$ 4.3} & 41.6 \scriptsize{$\pm$ 2.5} & 70.4 \scriptsize{$\pm$ 0.9} & 43.9 \scriptsize{$\pm$ 2.5} & 17.6 \scriptsize{$\pm$ 3.3} & 39.7 \scriptsize{$\pm$ 4.2} & 47.1 \scriptsize{$\pm$ 2.6} & 32.2 \scriptsize{$\pm$ 5.3} & 17.6 \scriptsize{$\pm$ 1.2} & \textbf{22.0} \scriptsize{$\pm$ 0.8} & 89.6 \scriptsize{$\pm$ 2.1} & 65.0 \scriptsize{$\pm$ 4.7} & 65.5 \scriptsize{$\pm$ 10.3} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
79.2 \scriptsize{$\pm$ 0.8} & 26.2 \scriptsize{$\pm$ 3.0} & 12.6 \scriptsize{$\pm$ 0.7} & 59.6 \scriptsize{$\pm$ 2.4} & 50.6 \scriptsize{$\pm$ 3.9} & 41.9 \scriptsize{$\pm$ 2.4} & 69.2 \scriptsize{$\pm$ 1.7} & 44.3 \scriptsize{$\pm$ 2.3} & 17.6 \scriptsize{$\pm$ 3.2} & 39.7 \scriptsize{$\pm$ 4.1} & \textbf{47.3} \scriptsize{$\pm$ 2.7} & \textbf{33.6} \scriptsize{$\pm$ 4.7} & 18.0 \scriptsize{$\pm$ 1.2} & 21.9 \scriptsize{$\pm$ 0.8} & \textbf{90.9} \scriptsize{$\pm$ 1.8} & 68.4 \scriptsize{$\pm$ 4.4} & \textbf{68.6} \scriptsize{$\pm$ 8.4} \cr
DeFRCN~\cite{qiao2021defrcn} &
\textbf{79.6} \scriptsize{$\pm$ 0.5} & 24.5 \scriptsize{$\pm$ 1.7} & 9.6 \scriptsize{$\pm$ 0.4} & \textbf{64.8} \scriptsize{$\pm$ 3.9} & 48.3 \scriptsize{$\pm$ 2.2} & \textbf{44.3} \scriptsize{$\pm$ 2.7} & 66.4 \scriptsize{$\pm$ 2.6} & 39.4 \scriptsize{$\pm$ 3.3} & 20.1 \scriptsize{$\pm$ 3.1} & 30.7 \scriptsize{$\pm$ 4.2} & 44.7 \scriptsize{$\pm$ 1.9} & 22.4 \scriptsize{$\pm$ 4.9} & 17.5 \scriptsize{$\pm$ 1.4} & 19.4 \scriptsize{$\pm$ 1.1} & 89.4 \scriptsize{$\pm$ 1.1} & 70.7 \scriptsize{$\pm$ 3.1} & 60.8 \scriptsize{$\pm$ 6.3} \cr
\rowcolor{Gray} FT &
79.2 \scriptsize{$\pm$ 0.6} & \textbf{28.7} \scriptsize{$\pm$ 2.8} & \textbf{13.5} \scriptsize{$\pm$ 0.6} & 60.4 \scriptsize{$\pm$ 2.5} & \textbf{52.1} \scriptsize{$\pm$ 5.3} & 40.3 \scriptsize{$\pm$ 2.6} & 68.2 \scriptsize{$\pm$ 3.3} & \textbf{51.0} \scriptsize{$\pm$ 2.9} & \textbf{22.0} \scriptsize{$\pm$ 4.1} & 33.8 \scriptsize{$\pm$ 2.8} & 46.4 \scriptsize{$\pm$ 1.5} & 32.1 \scriptsize{$\pm$ 3.9} & \textbf{19.8} \scriptsize{$\pm$ 1.5} & 21.4 \scriptsize{$\pm$ 0.8} & 88.8 \scriptsize{$\pm$ 1.9} & \textbf{76.9} \scriptsize{$\pm$ 4.0} & 62.9 \scriptsize{$\pm$ 9.5} \cr
\midrule
\multirowcell{2}{5-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
& LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
16.1 \scriptsize{$\pm$ 3.7} & 4.9 \scriptsize{$\pm$ 0.9} & 2.3 \scriptsize{$\pm$ 0.4} & 0.5 \scriptsize{$\pm$ 0.4} & 31.1 \scriptsize{$\pm$ 1.1} & 60.9 \scriptsize{$\pm$ 1.9} & 8.3 \scriptsize{$\pm$ 1.0} & 8.4 \scriptsize{$\pm$ 1.9} & 19.0 \scriptsize{$\pm$ 4.9} & 0.3 \scriptsize{$\pm$ 0.3} & 46.0 \scriptsize{$\pm$ 4.1} & 48.3 \scriptsize{$\pm$ 4.4} & 39.9 \scriptsize{$\pm$ 3.8} & 7.4 \scriptsize{$\pm$ 1.0} & 8.8 \scriptsize{$\pm$ 1.7} & 27.9 \scriptsize{$\pm$ 1.7} & 4.7 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
12.5 \scriptsize{$\pm$ 3.3} & 4.0 \scriptsize{$\pm$ 0.8} & 2.2 \scriptsize{$\pm$ 0.5} & 0.5 \scriptsize{$\pm$ 0.5} & 31.8 \scriptsize{$\pm$ 1.1} & \textbf{61.2} \scriptsize{$\pm$ 1.9} & 8.3 \scriptsize{$\pm$ 1.0} & 8.6 \scriptsize{$\pm$ 1.9} & 19.3 \scriptsize{$\pm$ 5.1} & 0.4 \scriptsize{$\pm$ 0.3} & \textbf{47.1} \scriptsize{$\pm$ 4.3} & \textbf{49.2} \scriptsize{$\pm$ 3.7} & 40.4 \scriptsize{$\pm$ 4.7} & 6.2 \scriptsize{$\pm$ 1.1} & 8.5 \scriptsize{$\pm$ 1.5} & 27.7 \scriptsize{$\pm$ 1.7} & 4.7 \scriptsize{$\pm$ 0.4} \cr
FSCE-base~\cite{sun2021fsce} &
46.0 \scriptsize{$\pm$ 3.5} & 19.7 \scriptsize{$\pm$ 1.8} & 5.7 \scriptsize{$\pm$ 0.9} & 0.6 \scriptsize{$\pm$ 0.5} & \textbf{51.5} \scriptsize{$\pm$ 2.2} & 56.3 \scriptsize{$\pm$ 2.1} & 15.0 \scriptsize{$\pm$ 1.8} & 14.9 \scriptsize{$\pm$ 2.5} & 27.3 \scriptsize{$\pm$ 7.3} & 4.1 \scriptsize{$\pm$ 2.3} & 40.2 \scriptsize{$\pm$ 4.4} & 47.0 \scriptsize{$\pm$ 4.5} & 53.2 \scriptsize{$\pm$ 4.1} & \textbf{28.4} \scriptsize{$\pm$ 3.1} & 24.4 \scriptsize{$\pm$ 3.0} & 37.9 \scriptsize{$\pm$ 2.0} & 2.9 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
43.3 \scriptsize{$\pm$ 3.5} & 20.1 \scriptsize{$\pm$ 2.1} & 5.8 \scriptsize{$\pm$ 0.8} & 0.7 \scriptsize{$\pm$ 0.6} & 51.1 \scriptsize{$\pm$ 2.0} & 55.9 \scriptsize{$\pm$ 2.0} & 16.0 \scriptsize{$\pm$ 1.8} & 15.7 \scriptsize{$\pm$ 2.8} & 27.8 \scriptsize{$\pm$ 7.7} & 4.3 \scriptsize{$\pm$ 2.5} & 39.5 \scriptsize{$\pm$ 4.0} & 47.2 \scriptsize{$\pm$ 4.6} & \textbf{56.3} \scriptsize{$\pm$ 3.5} & 21.4 \scriptsize{$\pm$ 3.7} & 25.0 \scriptsize{$\pm$ 2.9} & 38.1 \scriptsize{$\pm$ 1.8} & 2.7 \scriptsize{$\pm$ 0.3} \cr
DeFRCN~\cite{qiao2021defrcn} &
46.3 \scriptsize{$\pm$ 3.8} & 19.3 \scriptsize{$\pm$ 3.0} & 4.5 \scriptsize{$\pm$ 0.8} & 0.1 \scriptsize{$\pm$ 0.3} & 45.7 \scriptsize{$\pm$ 2.5} & 57.5 \scriptsize{$\pm$ 1.4} & \textbf{25.1} \scriptsize{$\pm$ 1.4} & \textbf{22.4} \scriptsize{$\pm$ 2.7} & 40.9 \scriptsize{$\pm$ 9.8} & 1.4 \scriptsize{$\pm$ 1.1} & 39.0 \scriptsize{$\pm$ 4.1} & 44.2 \scriptsize{$\pm$ 4.0} & 43.2 \scriptsize{$\pm$ 4.8} & 7.8 \scriptsize{$\pm$ 1.5} & 25.4 \scriptsize{$\pm$ 3.3} & 36.7 \scriptsize{$\pm$ 1.9} & 3.5 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} FT &
\textbf{49.0} \scriptsize{$\pm$ 3.6} & \textbf{22.3} \scriptsize{$\pm$ 3.2} & \textbf{6.8} \scriptsize{$\pm$ 1.3} & \textbf{1.4} \scriptsize{$\pm$ 0.5} & 49.9 \scriptsize{$\pm$ 2.0} & 56.0 \scriptsize{$\pm$ 2.2} & 23.5 \scriptsize{$\pm$ 2.2} & 22.1 \scriptsize{$\pm$ 3.5} & \textbf{46.7} \scriptsize{$\pm$ 12.4} & \textbf{5.3} \scriptsize{$\pm$ 3.5} & 39.2 \scriptsize{$\pm$ 3.8} & 43.0 \scriptsize{$\pm$ 3.6} & 49.4 \scriptsize{$\pm$ 3.2} & 24.7 \scriptsize{$\pm$ 3.1} & \textbf{30.8} \scriptsize{$\pm$ 3.3} & \textbf{39.6} \scriptsize{$\pm$ 2.3} & \textbf{2.4} \scriptsize{$\pm$ 0.5} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{ccccccccccccccccccccccccc}
\toprule
\multirowcell{2}{10-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
& CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
73.4 \scriptsize{$\pm$ 0.5} & 13.1 \scriptsize{$\pm$ 1.3} & 10.3 \scriptsize{$\pm$ 0.5} & 58.6 \scriptsize{$\pm$ 1.4} & 46.1 \scriptsize{$\pm$ 1.5} & 36.2 \scriptsize{$\pm$ 2.7} & 74.3 \scriptsize{$\pm$ 2.2} & 48.6 \scriptsize{$\pm$ 0.5} & 22.1 \scriptsize{$\pm$ 3.7} & \textbf{44.3} \scriptsize{$\pm$ 4.6} & 41.6 \scriptsize{$\pm$ 1.6} & 2.0 \scriptsize{$\pm$ 0.6} & 10.5 \scriptsize{$\pm$ 0.9} & 8.9 \scriptsize{$\pm$ 1.2} & 78.1 \scriptsize{$\pm$ 1.4} & 44.3 \scriptsize{$\pm$ 1.5} & 36.6 \scriptsize{$\pm$ 5.6} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
72.9 \scriptsize{$\pm$ 0.6} & 13.1 \scriptsize{$\pm$ 1.3} & 10.4 \scriptsize{$\pm$ 0.4} & 56.1 \scriptsize{$\pm$ 1.7} & 46.7 \scriptsize{$\pm$ 1.3} & 35.2 \scriptsize{$\pm$ 2.6} & \textbf{74.6} \scriptsize{$\pm$ 1.8} & 47.9 \scriptsize{$\pm$ 0.9} & 22.1 \scriptsize{$\pm$ 3.6} & 44.0 \scriptsize{$\pm$ 4.3} & 41.8 \scriptsize{$\pm$ 1.5} & 2.1 \scriptsize{$\pm$ 0.7} & 10.5 \scriptsize{$\pm$ 1.0} & 8.3 \scriptsize{$\pm$ 0.9} & 77.9 \scriptsize{$\pm$ 1.3} & 40.2 \scriptsize{$\pm$ 1.9} & 37.7 \scriptsize{$\pm$ 5.8} \cr
FSCE-base~\cite{sun2021fsce} &
80.0 \scriptsize{$\pm$ 0.0} & 35.6 \scriptsize{$\pm$ 2.5} & 14.8 \scriptsize{$\pm$ 0.6} & 69.4 \scriptsize{$\pm$ 2.0} & 56.0 \scriptsize{$\pm$ 3.0} & 53.2 \scriptsize{$\pm$ 2.4} & 72.5 \scriptsize{$\pm$ 1.8} & 51.1 \scriptsize{$\pm$ 1.3} & 20.7 \scriptsize{$\pm$ 4.1} & 42.0 \scriptsize{$\pm$ 5.0} & 51.1 \scriptsize{$\pm$ 1.8} & 38.0 \scriptsize{$\pm$ 5.4} & 22.5 \scriptsize{$\pm$ 1.1} & 24.3 \scriptsize{$\pm$ 1.1} & 91.5 \scriptsize{$\pm$ 1.0} & 79.3 \scriptsize{$\pm$ 2.3} & 75.9 \scriptsize{$\pm$ 3.4} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
79.9 \scriptsize{$\pm$ 0.3} & 35.9 \scriptsize{$\pm$ 2.5} & 15.0 \scriptsize{$\pm$ 0.5} & 69.9 \scriptsize{$\pm$ 2.0} & 56.3 \scriptsize{$\pm$ 3.1} & 52.9 \scriptsize{$\pm$ 1.9} & 71.4 \scriptsize{$\pm$ 2.0} & 51.4 \scriptsize{$\pm$ 0.9} & 20.8 \scriptsize{$\pm$ 4.0} & 42.6 \scriptsize{$\pm$ 4.6} & \textbf{51.2} \scriptsize{$\pm$ 1.8} & \textbf{38.8} \scriptsize{$\pm$ 5.0} & 23.2 \scriptsize{$\pm$ 1.1} & 24.3 \scriptsize{$\pm$ 0.8} & \textbf{92.9} \scriptsize{$\pm$ 0.7} & 82.3 \scriptsize{$\pm$ 2.8} & \textbf{77.4} \scriptsize{$\pm$ 3.7} \cr
DeFRCN~\cite{qiao2021defrcn} &
\textbf{80.1} \scriptsize{$\pm$ 0.4} & 31.1 \scriptsize{$\pm$ 2.2} & 10.8 \scriptsize{$\pm$ 0.5} & \textbf{73.6} \scriptsize{$\pm$ 2.6} & 53.0 \scriptsize{$\pm$ 1.9} & 53.6 \scriptsize{$\pm$ 2.9} & 67.8 \scriptsize{$\pm$ 3.0} & 47.6 \scriptsize{$\pm$ 1.5} & 24.3 \scriptsize{$\pm$ 4.7} & 34.1 \scriptsize{$\pm$ 4.2} & 48.5 \scriptsize{$\pm$ 1.6} & 27.1 \scriptsize{$\pm$ 2.5} & 21.6 \scriptsize{$\pm$ 1.1} & 20.7 \scriptsize{$\pm$ 1.4} & 90.9 \scriptsize{$\pm$ 1.0} & 78.3 \scriptsize{$\pm$ 2.4} & 68.4 \scriptsize{$\pm$ 3.2} \cr
\rowcolor{Gray} FT &
79.8 \scriptsize{$\pm$ 0.1} & \textbf{39.5} \scriptsize{$\pm$ 3.7} & \textbf{16.8} \scriptsize{$\pm$ 0.9} & 71.8 \scriptsize{$\pm$ 1.7} & \textbf{57.2} \scriptsize{$\pm$ 4.8} & \textbf{55.1} \scriptsize{$\pm$ 2.6} & 70.9 \scriptsize{$\pm$ 3.1} & \textbf{59.2} \scriptsize{$\pm$ 1.1} & \textbf{25.7} \scriptsize{$\pm$ 5.3} & 39.0 \scriptsize{$\pm$ 4.1} & 50.3 \scriptsize{$\pm$ 1.7} & 36.5 \scriptsize{$\pm$ 4.4} & \textbf{24.9} \scriptsize{$\pm$ 1.5} & \textbf{24.5} \scriptsize{$\pm$ 0.8} & 90.9 \scriptsize{$\pm$ 1.0} & \textbf{88.9} \scriptsize{$\pm$ 1.7} & 73.3 \scriptsize{$\pm$ 5.1} \cr
\midrule
\multirowcell{2}{10-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
& LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
TFA-fc~\cite{wang2020frustratingly} &
17.9 \scriptsize{$\pm$ 4.5} & 5.0 \scriptsize{$\pm$ 1.1} & 3.0 \scriptsize{$\pm$ 0.4} & 0.8 \scriptsize{$\pm$ 0.5} & 32.2 \scriptsize{$\pm$ 1.0} & 63.5 \scriptsize{$\pm$ 1.1} & 13.4 \scriptsize{$\pm$ 1.5} & 12.2 \scriptsize{$\pm$ 2.0} & 29.2 \scriptsize{$\pm$ 3.2} & 0.4 \scriptsize{$\pm$ 0.3} & 47.7 \scriptsize{$\pm$ 2.6} & 53.8 \scriptsize{$\pm$ 2.2} & 43.2 \scriptsize{$\pm$ 3.2} & 8.0 \scriptsize{$\pm$ 1.1} & 10.7 \scriptsize{$\pm$ 1.0} & 30.9 \scriptsize{$\pm$ 1.3} & 4.7 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} TFA-cos~\cite{wang2020frustratingly} &
12.8 \scriptsize{$\pm$ 3.6} & 3.8 \scriptsize{$\pm$ 1.0} & 2.9 \scriptsize{$\pm$ 0.4} & 1.0 \scriptsize{$\pm$ 0.4} & 32.9 \scriptsize{$\pm$ 1.0} & \textbf{63.6} \scriptsize{$\pm$ 1.1} & 12.9 \scriptsize{$\pm$ 1.5} & 12.1 \scriptsize{$\pm$ 2.0} & 29.0 \scriptsize{$\pm$ 2.8} & 0.4 \scriptsize{$\pm$ 0.1} & \textbf{48.5} \scriptsize{$\pm$ 2.6} & \textbf{54.0} \scriptsize{$\pm$ 2.1} & 43.1 \scriptsize{$\pm$ 2.9} & 6.6 \scriptsize{$\pm$ 1.0} & 10.2 \scriptsize{$\pm$ 0.9} & 30.5 \scriptsize{$\pm$ 1.3} & 4.8 \scriptsize{$\pm$ 0.4} \cr
FSCE-base~\cite{sun2021fsce} &
55.0 \scriptsize{$\pm$ 4.4} & 25.5 \scriptsize{$\pm$ 1.7} & 8.7 \scriptsize{$\pm$ 0.9} & 0.9 \scriptsize{$\pm$ 0.5} & \textbf{54.0} \scriptsize{$\pm$ 1.5} & 58.7 \scriptsize{$\pm$ 1.5} & 24.5 \scriptsize{$\pm$ 3.7} & 22.0 \scriptsize{$\pm$ 2.4} & 34.6 \scriptsize{$\pm$ 6.8} & 9.0 \scriptsize{$\pm$ 1.9} & 44.2 \scriptsize{$\pm$ 2.4} & 53.9 \scriptsize{$\pm$ 2.5} & 60.7 \scriptsize{$\pm$ 4.5} & \textbf{28.5} \scriptsize{$\pm$ 4.2} & 31.4 \scriptsize{$\pm$ 2.2} & 43.4 \scriptsize{$\pm$ 1.6} & 2.8 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} FSCE-con~\cite{sun2021fsce} &
47.3 \scriptsize{$\pm$ 4.2} & 22.9 \scriptsize{$\pm$ 2.3} & 8.5 \scriptsize{$\pm$ 0.6} & 1.1 \scriptsize{$\pm$ 0.5} & 53.6 \scriptsize{$\pm$ 1.4} & 58.4 \scriptsize{$\pm$ 1.5} & 26.5 \scriptsize{$\pm$ 3.5} & 23.1 \scriptsize{$\pm$ 2.1} & 36.0 \scriptsize{$\pm$ 6.5} & 9.2 \scriptsize{$\pm$ 1.6} & 43.0 \scriptsize{$\pm$ 2.3} & 53.9 \scriptsize{$\pm$ 2.5} & \textbf{63.2} \scriptsize{$\pm$ 4.3} & 21.1 \scriptsize{$\pm$ 3.4} & 32.1 \scriptsize{$\pm$ 2.3} & 43.3 \scriptsize{$\pm$ 1.5} & 2.7 \scriptsize{$\pm$ 0.3} \cr
DeFRCN~\cite{qiao2021defrcn} &
51.5 \scriptsize{$\pm$ 3.9} & 22.5 \scriptsize{$\pm$ 2.0} & 6.7 \scriptsize{$\pm$ 0.7} & 0.5 \scriptsize{$\pm$ 0.5} & 47.6 \scriptsize{$\pm$ 1.6} & 60.4 \scriptsize{$\pm$ 1.0} & 33.7 \scriptsize{$\pm$ 2.0} & 30.8 \scriptsize{$\pm$ 1.5} & 48.4 \scriptsize{$\pm$ 11.1} & 3.2 \scriptsize{$\pm$ 1.4} & 42.0 \scriptsize{$\pm$ 1.8} & 49.5 \scriptsize{$\pm$ 2.7} & 49.6 \scriptsize{$\pm$ 2.7} & 8.6 \scriptsize{$\pm$ 1.7} & 33.4 \scriptsize{$\pm$ 3.1} & 41.2 \scriptsize{$\pm$ 1.9} & 3.7 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} FT &
\textbf{60.0} \scriptsize{$\pm$ 5.1} & \textbf{27.7} \scriptsize{$\pm$ 2.0} & \textbf{10.9} \scriptsize{$\pm$ 0.7} & \textbf{2.1} \scriptsize{$\pm$ 0.9} & 52.0 \scriptsize{$\pm$ 1.4} & 57.2 \scriptsize{$\pm$ 1.8} & \textbf{35.1} \scriptsize{$\pm$ 3.4} & \textbf{35.2} \scriptsize{$\pm$ 2.2} & \textbf{53.5} \scriptsize{$\pm$ 11.1} & \textbf{10.6} \scriptsize{$\pm$ 1.5} & 42.0 \scriptsize{$\pm$ 3.1} & 49.8 \scriptsize{$\pm$ 2.6} & 57.8 \scriptsize{$\pm$ 4.2} & 25.9 \scriptsize{$\pm$ 4.1} & \textbf{40.6} \scriptsize{$\pm$ 3.0} & \textbf{45.8} \scriptsize{$\pm$ 2.1} & \textbf{2.2} \scriptsize{$\pm$ 0.5} \cr
\bottomrule
\end{tabular}
}
\caption{
Performance of methods on all 32 datasets in the proposed benchmark.
}
\label{tb:result_32}
\end{sidewaystable*}


==> table_arch_32.tex <==
\begin{sidewaystable*}[t]
\def\smidrulea{\cmidrule(rl){1-2}\cmidrule(rl){3-5}\cmidrule(rl){6-7}\cmidrule(rl){8-9}\cmidrule(rl){10-12}\cmidrule(rl){13-13}\cmidrule(rl){14-14}\cmidrule(rl){15-16}\cmidrule(rl){17-18}\cmidrule(rl){19-19}}
\def\smidruleb{\cmidrule(rl){1-2}\cmidrule(rl){3-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(rl){9-10}\cmidrule(rl){11-11}\cmidrule(rl){12-12}\cmidrule(rl){13-16}\cmidrule(rl){17-17}}
\def\smidrulec{\cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}\cmidrule(rl){6-6}\cmidrule(rl){7-7}\cmidrule(rl){8-8}\cmidrule(rl){9-9}\cmidrule(rl){10-10}\cmidrule(rl){11-11}\cmidrule(rl){12-12}\cmidrule(rl){13-13}\cmidrule(rl){14-14}\cmidrule(rl){15-15}\cmidrule(rl){16-16}\cmidrule(rl){17-17}\cmidrule(rl){18-18}\cmidrule(rl){19-19}}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccccccccccc}
\toprule
\multicolumn{2}{c}{1-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
Arch & Pre-train & CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
FRCN & COCO &
76.0 \scriptsize{$\pm$ 3.0} & 13.8 \scriptsize{$\pm$ 2.5} & 7.7 \scriptsize{$\pm$ 0.7} & 33.8 \scriptsize{$\pm$ 8.1} & 33.0 \scriptsize{$\pm$ 7.6} & 18.4 \scriptsize{$\pm$ 1.6} & \textbf{60.5} \scriptsize{$\pm$ 5.3} & \textbf{34.9} \scriptsize{$\pm$ 4.6} & \textbf{21.4} \scriptsize{$\pm$ 5.3} & \textbf{32.2} \scriptsize{$\pm$ 4.1} & 35.4 \scriptsize{$\pm$ 8.5} & 11.7 \scriptsize{$\pm$ 7.6} & 9.7 \scriptsize{$\pm$ 2.2} & 12.9 \scriptsize{$\pm$ 1.1} & 71.2 \scriptsize{$\pm$ 8.1} & 43.0 \scriptsize{$\pm$ 6.6} & 33.0 \scriptsize{$\pm$ 17.2} \cr
\rowcolor{Gray} & COCO &
\textbf{76.8} \scriptsize{$\pm$ 2.2} & 15.0 \scriptsize{$\pm$ 2.8} & 8.9 \scriptsize{$\pm$ 1.1} & 38.3 \scriptsize{$\pm$ 5.3} & 32.8 \scriptsize{$\pm$ 12.3} & 18.9 \scriptsize{$\pm$ 2.4} & 36.9 \scriptsize{$\pm$ 12.7} & 28.1 \scriptsize{$\pm$ 3.6} & 18.6 \scriptsize{$\pm$ 3.5} & 23.3 \scriptsize{$\pm$ 2.5} & \textbf{36.3} \scriptsize{$\pm$ 6.3} & 10.9 \scriptsize{$\pm$ 6.5} & 11.4 \scriptsize{$\pm$ 1.4} & 14.3 \scriptsize{$\pm$ 1.2} & 80.1 \scriptsize{$\pm$ 6.5} & 51.8 \scriptsize{$\pm$ 6.6} & 26.1 \scriptsize{$\pm$ 12.6} \cr
\rowcolor{Gray} & FSODD &
71.2 \scriptsize{$\pm$ 5.5} & 12.7 \scriptsize{$\pm$ 2.8} & 5.8 \scriptsize{$\pm$ 0.4} & 47.9 \scriptsize{$\pm$ 3.3} & 32.2 \scriptsize{$\pm$ 11.3} & \textbf{26.0} \scriptsize{$\pm$ 2.7} & 41.3 \scriptsize{$\pm$ 10.4} & 12.6 \scriptsize{$\pm$ 2.3} & 11.8 \scriptsize{$\pm$ 2.5} & 17.7 \scriptsize{$\pm$ 3.2} & 29.9 \scriptsize{$\pm$ 5.5} & 8.8 \scriptsize{$\pm$ 6.1} & \textbf{13.5} \scriptsize{$\pm$ 2.1} & 14.9 \scriptsize{$\pm$ 1.1} & 77.2 \scriptsize{$\pm$ 6.4} & 52.4 \scriptsize{$\pm$ 6.5} & 31.7 \scriptsize{$\pm$ 12.2} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
76.5 \scriptsize{$\pm$ 3.1} & \textbf{16.7} \scriptsize{$\pm$ 2.7} & \textbf{9.9} \scriptsize{$\pm$ 1.0} & \textbf{48.0} \scriptsize{$\pm$ 5.7} & \textbf{37.7} \scriptsize{$\pm$ 11.4} & 24.3 \scriptsize{$\pm$ 2.8} & 44.4 \scriptsize{$\pm$ 9.7} & 31.8 \scriptsize{$\pm$ 5.2} & 21.2 \scriptsize{$\pm$ 2.9} & 28.2 \scriptsize{$\pm$ 3.3} & 35.8 \scriptsize{$\pm$ 8.6} & \textbf{21.5} \scriptsize{$\pm$ 5.5} & 13.3 \scriptsize{$\pm$ 2.1} & \textbf{18.4} \scriptsize{$\pm$ 1.5} & \textbf{81.5} \scriptsize{$\pm$ 5.4} & \textbf{53.5} \scriptsize{$\pm$ 5.5} & \textbf{36.1} \scriptsize{$\pm$ 12.3} \cr
\bottomrule
\multicolumn{2}{c}{1-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
Arch & Pre-train & LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
FRCN & COCO &
23.2 \scriptsize{$\pm$ 4.5} & 9.7 \scriptsize{$\pm$ 1.3} & 3.2 \scriptsize{$\pm$ 0.9} & 0.5 \scriptsize{$\pm$ 0.3} & 43.7 \scriptsize{$\pm$ 4.4} & \textbf{51.1} \scriptsize{$\pm$ 6.8} & 8.1 \scriptsize{$\pm$ 2.8} & 6.9 \scriptsize{$\pm$ 3.7} & 15.1 \scriptsize{$\pm$ 6.4} & 1.4 \scriptsize{$\pm$ 1.2} & 29.9 \scriptsize{$\pm$ 3.1} & 38.6 \scriptsize{$\pm$ 5.4} & 27.2 \scriptsize{$\pm$ 5.1} & 15.2 \scriptsize{$\pm$ 2.1} & 16.0 \scriptsize{$\pm$ 2.5} & 26.2 \scriptsize{$\pm$ 3.3} & 2.8 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} & COCO &
28.9 \scriptsize{$\pm$ 4.6} & 12.5 \scriptsize{$\pm$ 1.5} & 3.1 \scriptsize{$\pm$ 1.2} & 0.4 \scriptsize{$\pm$ 0.3} & 44.5 \scriptsize{$\pm$ 3.4} & 49.9 \scriptsize{$\pm$ 7.4} & 10.7 \scriptsize{$\pm$ 2.8} & 7.3 \scriptsize{$\pm$ 3.7} & \textbf{20.7} \scriptsize{$\pm$ 6.4} & 1.7 \scriptsize{$\pm$ 1.2} & 30.8 \scriptsize{$\pm$ 2.3} & 39.7 \scriptsize{$\pm$ 3.2} & 31.8 \scriptsize{$\pm$ 6.1} & 15.5 \scriptsize{$\pm$ 2.0} & 18.8 \scriptsize{$\pm$ 2.3} & 26.4 \scriptsize{$\pm$ 3.3} & 2.5 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} & FSODD &
29.8 \scriptsize{$\pm$ 4.6} & 11.4 \scriptsize{$\pm$ 1.6} & 2.6 \scriptsize{$\pm$ 1.1} & 0.5 \scriptsize{$\pm$ 0.5} & 28.3 \scriptsize{$\pm$ 1.6} & 28.0 \scriptsize{$\pm$ 10.1} & 11.0 \scriptsize{$\pm$ 2.9} & 8.2 \scriptsize{$\pm$ 3.7} & 18.9 \scriptsize{$\pm$ 7.6} & \textbf{1.8} \scriptsize{$\pm$ 1.1} & 15.2 \scriptsize{$\pm$ 1.8} & 25.0 \scriptsize{$\pm$ 3.1} & 26.3 \scriptsize{$\pm$ 4.9} & 13.7 \scriptsize{$\pm$ 1.6} & 17.3 \scriptsize{$\pm$ 2.6} & 23.3 \scriptsize{$\pm$ 3.2} & 3.0 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{31.2} \scriptsize{$\pm$ 5.3} & \textbf{13.7} \scriptsize{$\pm$ 1.9} & \textbf{3.7} \scriptsize{$\pm$ 1.1} & \textbf{0.6} \scriptsize{$\pm$ 0.4} & \textbf{46.0} \scriptsize{$\pm$ 3.0} & 46.8 \scriptsize{$\pm$ 8.0} & \textbf{11.7} \scriptsize{$\pm$ 3.4} & \textbf{10.8} \scriptsize{$\pm$ 4.8} & 20.2 \scriptsize{$\pm$ 5.9} & 1.6 \scriptsize{$\pm$ 1.3} & \textbf{32.7} \scriptsize{$\pm$ 3.2} & \textbf{40.1} \scriptsize{$\pm$ 3.9} & \textbf{37.5} \scriptsize{$\pm$ 5.3} & \textbf{17.9} \scriptsize{$\pm$ 2.2} & \textbf{20.0} \scriptsize{$\pm$ 2.2} & \textbf{29.2} \scriptsize{$\pm$ 2.9} & \textbf{1.6} \scriptsize{$\pm$ 0.4} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{ccccccccccccccccccc}
\toprule
\multicolumn{2}{c}{3-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
Arch & Pre-train & CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
FRCN & COCO &
78.9 \scriptsize{$\pm$ 0.6} & 22.0 \scriptsize{$\pm$ 2.6} & 11.4 \scriptsize{$\pm$ 0.7} & 52.4 \scriptsize{$\pm$ 4.3} & 43.6 \scriptsize{$\pm$ 9.8} & 30.6 \scriptsize{$\pm$ 1.8} & \textbf{67.5} \scriptsize{$\pm$ 3.5} & \textbf{44.6} \scriptsize{$\pm$ 3.9} & 19.0 \scriptsize{$\pm$ 4.5} & \textbf{32.7} \scriptsize{$\pm$ 3.9} & 43.5 \scriptsize{$\pm$ 3.1} & 26.3 \scriptsize{$\pm$ 4.9} & 16.7 \scriptsize{$\pm$ 1.6} & 18.9 \scriptsize{$\pm$ 1.1} & 86.7 \scriptsize{$\pm$ 2.8} & 64.7 \scriptsize{$\pm$ 7.2} & 53.1 \scriptsize{$\pm$ 17.1} \cr
\rowcolor{Gray} & COCO &
79.7 \scriptsize{$\pm$ 0.5} & 23.0 \scriptsize{$\pm$ 2.8} & 12.8 \scriptsize{$\pm$ 0.8} & 53.5 \scriptsize{$\pm$ 3.7} & 43.4 \scriptsize{$\pm$ 9.8} & 32.5 \scriptsize{$\pm$ 2.0} & 62.5 \scriptsize{$\pm$ 5.7} & 35.8 \scriptsize{$\pm$ 2.0} & 18.4 \scriptsize{$\pm$ 4.4} & 27.5 \scriptsize{$\pm$ 6.0} & 42.0 \scriptsize{$\pm$ 5.9} & 26.7 \scriptsize{$\pm$ 4.3} & 18.5 \scriptsize{$\pm$ 1.0} & 19.5 \scriptsize{$\pm$ 0.8} & 88.9 \scriptsize{$\pm$ 2.3} & 71.5 \scriptsize{$\pm$ 4.7} & 49.0 \scriptsize{$\pm$ 12.2} \cr
\rowcolor{Gray} & FSODD &
78.3 \scriptsize{$\pm$ 1.2} & 20.1 \scriptsize{$\pm$ 2.5} & 8.9 \scriptsize{$\pm$ 0.7} & 61.7 \scriptsize{$\pm$ 3.4} & 42.8 \scriptsize{$\pm$ 8.0} & 37.0 \scriptsize{$\pm$ 2.3} & 62.6 \scriptsize{$\pm$ 4.8} & 19.7 \scriptsize{$\pm$ 2.6} & 12.4 \scriptsize{$\pm$ 1.8} & 20.5 \scriptsize{$\pm$ 4.2} & 37.7 \scriptsize{$\pm$ 4.7} & 20.4 \scriptsize{$\pm$ 4.8} & 20.1 \scriptsize{$\pm$ 1.3} & 19.3 \scriptsize{$\pm$ 0.7} & 86.9 \scriptsize{$\pm$ 2.8} & 72.1 \scriptsize{$\pm$ 5.4} & 51.6 \scriptsize{$\pm$ 9.9} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{80.1} \scriptsize{$\pm$ 0.4} & \textbf{24.8} \scriptsize{$\pm$ 2.1} & \textbf{14.0} \scriptsize{$\pm$ 0.9} & \textbf{62.9} \scriptsize{$\pm$ 5.0} & \textbf{46.5} \scriptsize{$\pm$ 9.5} & \textbf{38.3} \scriptsize{$\pm$ 2.6} & 63.5 \scriptsize{$\pm$ 4.6} & 42.3 \scriptsize{$\pm$ 2.5} & \textbf{22.3} \scriptsize{$\pm$ 3.9} & 32.2 \scriptsize{$\pm$ 6.0} & \textbf{45.8} \scriptsize{$\pm$ 4.5} & \textbf{35.9} \scriptsize{$\pm$ 3.8} & \textbf{21.4} \scriptsize{$\pm$ 1.3} & \textbf{24.1} \scriptsize{$\pm$ 0.8} & \textbf{90.1} \scriptsize{$\pm$ 2.0} & \textbf{73.2} \scriptsize{$\pm$ 6.6} & \textbf{56.9} \scriptsize{$\pm$ 12.0} \cr
\bottomrule
\multicolumn{2}{c}{3-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
Arch & Pre-train & LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
FRCN & COCO &
40.8 \scriptsize{$\pm$ 4.9} & 18.4 \scriptsize{$\pm$ 2.5} & 5.8 \scriptsize{$\pm$ 1.2} & 1.0 \scriptsize{$\pm$ 0.4} & 47.7 \scriptsize{$\pm$ 2.4} & 54.9 \scriptsize{$\pm$ 2.4} & 15.5 \scriptsize{$\pm$ 1.8} & 14.7 \scriptsize{$\pm$ 6.0} & \textbf{43.2} \scriptsize{$\pm$ 13.2} & 4.2 \scriptsize{$\pm$ 2.4} & 35.0 \scriptsize{$\pm$ 4.3} & 40.9 \scriptsize{$\pm$ 3.6} & 42.3 \scriptsize{$\pm$ 4.3} & 23.5 \scriptsize{$\pm$ 2.5} & 24.6 \scriptsize{$\pm$ 3.1} & 35.2 \scriptsize{$\pm$ 3.5} & 2.9 \scriptsize{$\pm$ 0.4} \cr
\rowcolor{Gray} & COCO &
45.1 \scriptsize{$\pm$ 3.8} & 21.3 \scriptsize{$\pm$ 2.5} & 6.3 \scriptsize{$\pm$ 1.1} & 0.8 \scriptsize{$\pm$ 0.6} & 49.5 \scriptsize{$\pm$ 2.1} & \textbf{56.2} \scriptsize{$\pm$ 3.0} & 17.7 \scriptsize{$\pm$ 2.1} & 15.9 \scriptsize{$\pm$ 4.8} & 42.2 \scriptsize{$\pm$ 8.2} & 6.0 \scriptsize{$\pm$ 3.3} & 35.2 \scriptsize{$\pm$ 2.2} & 42.8 \scriptsize{$\pm$ 2.9} & 48.1 \scriptsize{$\pm$ 3.8} & 20.6 \scriptsize{$\pm$ 2.2} & 29.0 \scriptsize{$\pm$ 3.6} & 35.7 \scriptsize{$\pm$ 2.6} & 2.5 \scriptsize{$\pm$ 0.2} \cr
\rowcolor{Gray} & FSODD &
47.1 \scriptsize{$\pm$ 4.9} & 21.5 \scriptsize{$\pm$ 2.4} & 5.7 \scriptsize{$\pm$ 1.0} & 1.0 \scriptsize{$\pm$ 0.5} & 34.9 \scriptsize{$\pm$ 2.5} & 38.4 \scriptsize{$\pm$ 7.8} & 17.0 \scriptsize{$\pm$ 2.3} & 16.5 \scriptsize{$\pm$ 5.3} & 39.1 \scriptsize{$\pm$ 10.2} & 5.7 \scriptsize{$\pm$ 2.5} & 19.1 \scriptsize{$\pm$ 1.5} & 28.5 \scriptsize{$\pm$ 2.9} & 41.1 \scriptsize{$\pm$ 5.4} & 19.0 \scriptsize{$\pm$ 1.9} & 28.6 \scriptsize{$\pm$ 3.5} & 32.4 \scriptsize{$\pm$ 2.5} & 3.1 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{49.6} \scriptsize{$\pm$ 3.7} & \textbf{25.1} \scriptsize{$\pm$ 3.0} & \textbf{6.7} \scriptsize{$\pm$ 1.3} & \textbf{1.0} \scriptsize{$\pm$ 0.6} & \textbf{50.4} \scriptsize{$\pm$ 2.3} & 54.6 \scriptsize{$\pm$ 3.1} & \textbf{20.5} \scriptsize{$\pm$ 2.5} & \textbf{20.0} \scriptsize{$\pm$ 5.2} & 41.1 \scriptsize{$\pm$ 8.6} & \textbf{6.9} \scriptsize{$\pm$ 3.6} & \textbf{38.7} \scriptsize{$\pm$ 2.4} & \textbf{42.9} \scriptsize{$\pm$ 2.9} & \textbf{51.3} \scriptsize{$\pm$ 5.3} & \textbf{25.0} \scriptsize{$\pm$ 2.0} & \textbf{31.1} \scriptsize{$\pm$ 3.1} & \textbf{38.7} \scriptsize{$\pm$ 2.6} & \textbf{1.4} \scriptsize{$\pm$ 0.3} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{ccccccccccccccccccc}
\toprule
\multicolumn{2}{c}{5-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
Arch & Pre-train & CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
FRCN & COCO &
79.2 \scriptsize{$\pm$ 0.6} & 28.7 \scriptsize{$\pm$ 2.8} & 13.5 \scriptsize{$\pm$ 0.6} & 60.4 \scriptsize{$\pm$ 2.5} & 52.1 \scriptsize{$\pm$ 5.3} & 40.3 \scriptsize{$\pm$ 2.6} & \textbf{68.2} \scriptsize{$\pm$ 3.3} & \textbf{51.0} \scriptsize{$\pm$ 2.9} & 22.0 \scriptsize{$\pm$ 4.1} & 33.8 \scriptsize{$\pm$ 2.8} & 46.4 \scriptsize{$\pm$ 1.5} & 32.1 \scriptsize{$\pm$ 3.9} & 19.8 \scriptsize{$\pm$ 1.5} & 21.4 \scriptsize{$\pm$ 0.8} & 88.8 \scriptsize{$\pm$ 1.9} & 76.9 \scriptsize{$\pm$ 4.0} & 62.9 \scriptsize{$\pm$ 9.5} \cr
\rowcolor{Gray} & COCO &
79.9 \scriptsize{$\pm$ 0.3} & 30.9 \scriptsize{$\pm$ 2.8} & 14.9 \scriptsize{$\pm$ 0.8} & 62.1 \scriptsize{$\pm$ 3.0} & 51.3 \scriptsize{$\pm$ 5.3} & 41.3 \scriptsize{$\pm$ 2.5} & 64.0 \scriptsize{$\pm$ 5.7} & 43.4 \scriptsize{$\pm$ 2.8} & 20.7 \scriptsize{$\pm$ 3.9} & 29.9 \scriptsize{$\pm$ 3.8} & 45.7 \scriptsize{$\pm$ 2.2} & 32.8 \scriptsize{$\pm$ 3.0} & 21.2 \scriptsize{$\pm$ 1.3} & 22.0 \scriptsize{$\pm$ 0.4} & 91.0 \scriptsize{$\pm$ 1.8} & 81.7 \scriptsize{$\pm$ 3.8} & 60.7 \scriptsize{$\pm$ 7.3} \cr
\rowcolor{Gray} & FSODD &
78.4 \scriptsize{$\pm$ 1.0} & 27.7 \scriptsize{$\pm$ 2.7} & 10.7 \scriptsize{$\pm$ 0.7} & 67.5 \scriptsize{$\pm$ 2.6} & 50.9 \scriptsize{$\pm$ 5.0} & 45.7 \scriptsize{$\pm$ 3.0} & 64.7 \scriptsize{$\pm$ 3.2} & 26.0 \scriptsize{$\pm$ 2.4} & 14.2 \scriptsize{$\pm$ 2.2} & 23.0 \scriptsize{$\pm$ 3.1} & 41.2 \scriptsize{$\pm$ 2.4} & 26.2 \scriptsize{$\pm$ 2.7} & 24.2 \scriptsize{$\pm$ 1.4} & 21.2 \scriptsize{$\pm$ 0.5} & 88.6 \scriptsize{$\pm$ 1.9} & 81.8 \scriptsize{$\pm$ 3.7} & 60.3 \scriptsize{$\pm$ 6.1} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{80.2} \scriptsize{$\pm$ 0.4} & \textbf{33.2} \scriptsize{$\pm$ 2.5} & \textbf{16.3} \scriptsize{$\pm$ 0.8} & \textbf{68.8} \scriptsize{$\pm$ 3.8} & \textbf{54.7} \scriptsize{$\pm$ 4.3} & \textbf{48.0} \scriptsize{$\pm$ 2.5} & 65.3 \scriptsize{$\pm$ 4.6} & 49.3 \scriptsize{$\pm$ 3.4} & \textbf{25.3} \scriptsize{$\pm$ 4.4} & \textbf{35.8} \scriptsize{$\pm$ 3.4} & \textbf{48.9} \scriptsize{$\pm$ 1.2} & \textbf{39.1} \scriptsize{$\pm$ 3.1} & \textbf{25.5} \scriptsize{$\pm$ 1.6} & \textbf{26.3} \scriptsize{$\pm$ 0.5} & \textbf{91.7} \scriptsize{$\pm$ 1.3} & \textbf{83.6} \scriptsize{$\pm$ 4.4} & \textbf{67.7} \scriptsize{$\pm$ 4.8} \cr
\bottomrule
\multicolumn{2}{c}{5-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
Arch & Pre-train & LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
FRCN & COCO &
49.0 \scriptsize{$\pm$ 3.6} & 22.3 \scriptsize{$\pm$ 3.2} & 6.8 \scriptsize{$\pm$ 1.3} & 1.4 \scriptsize{$\pm$ 0.5} & 49.9 \scriptsize{$\pm$ 2.0} & 56.0 \scriptsize{$\pm$ 2.2} & 23.5 \scriptsize{$\pm$ 2.2} & 22.1 \scriptsize{$\pm$ 3.5} & \textbf{46.7} \scriptsize{$\pm$ 12.4} & 5.3 \scriptsize{$\pm$ 3.5} & 39.2 \scriptsize{$\pm$ 3.8} & 43.0 \scriptsize{$\pm$ 3.6} & 49.4 \scriptsize{$\pm$ 3.2} & 24.7 \scriptsize{$\pm$ 3.1} & 30.8 \scriptsize{$\pm$ 3.3} & 39.6 \scriptsize{$\pm$ 2.3} & 3.0 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} & COCO &
53.9 \scriptsize{$\pm$ 4.1} & 25.6 \scriptsize{$\pm$ 2.9} & 8.0 \scriptsize{$\pm$ 1.5} & 1.2 \scriptsize{$\pm$ 0.6} & 51.6 \scriptsize{$\pm$ 1.8} & \textbf{57.7} \scriptsize{$\pm$ 2.1} & 26.0 \scriptsize{$\pm$ 1.7} & 23.1 \scriptsize{$\pm$ 3.9} & 45.8 \scriptsize{$\pm$ 10.0} & 7.1 \scriptsize{$\pm$ 4.7} & 38.2 \scriptsize{$\pm$ 3.5} & 45.2 \scriptsize{$\pm$ 3.9} & 55.4 \scriptsize{$\pm$ 2.7} & 23.8 \scriptsize{$\pm$ 3.4} & 35.0 \scriptsize{$\pm$ 2.8} & 40.3 \scriptsize{$\pm$ 2.0} & 2.5 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} & FSODD &
55.7 \scriptsize{$\pm$ 3.1} & 25.2 \scriptsize{$\pm$ 3.2} & 7.3 \scriptsize{$\pm$ 1.1} & 1.2 \scriptsize{$\pm$ 0.4} & 38.4 \scriptsize{$\pm$ 2.3} & 42.3 \scriptsize{$\pm$ 2.9} & 25.1 \scriptsize{$\pm$ 1.7} & 22.7 \scriptsize{$\pm$ 3.8} & 41.5 \scriptsize{$\pm$ 10.0} & 7.1 \scriptsize{$\pm$ 3.5} & 22.3 \scriptsize{$\pm$ 1.8} & 32.1 \scriptsize{$\pm$ 3.6} & 48.7 \scriptsize{$\pm$ 4.3} & 21.1 \scriptsize{$\pm$ 3.1} & 33.7 \scriptsize{$\pm$ 3.1} & 36.8 \scriptsize{$\pm$ 1.8} & 3.3 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{59.7} \scriptsize{$\pm$ 3.1} & \textbf{30.5} \scriptsize{$\pm$ 3.6} & \textbf{8.2} \scriptsize{$\pm$ 1.3} & \textbf{1.6} \scriptsize{$\pm$ 0.5} & \textbf{53.1} \scriptsize{$\pm$ 1.7} & 57.0 \scriptsize{$\pm$ 2.0} & \textbf{30.1} \scriptsize{$\pm$ 2.8} & \textbf{27.4} \scriptsize{$\pm$ 3.6} & 43.6 \scriptsize{$\pm$ 8.1} & \textbf{9.0} \scriptsize{$\pm$ 4.6} & \textbf{42.8} \scriptsize{$\pm$ 4.6} & \textbf{46.4} \scriptsize{$\pm$ 4.0} & \textbf{57.4} \scriptsize{$\pm$ 2.4} & \textbf{27.3} \scriptsize{$\pm$ 3.3} & \textbf{36.5} \scriptsize{$\pm$ 3.7} & \textbf{43.4} \scriptsize{$\pm$ 1.6} & \textbf{1.3} \scriptsize{$\pm$ 0.3} \cr
\bottomrule
\end{tabular}
}
\\
\resizebox{\linewidth}{!}{%
% \scalebox{0.8}{%
\begin{tabular}{ccccccccccccccccccc}
\toprule
\multicolumn{2}{c}{10-shot} & \multicolumn{3}{c}{Aerial} & \multicolumn{2}{c}{Agriculture} & \multicolumn{2}{c}{Animal} & \multicolumn{3}{c}{Cartoon} & Dense Product & Face & \multicolumn{2}{c}{Fashion} & \multicolumn{2}{c}{Food} & Head \cr \smidrulea
Arch & Pre-train & CARPK & DOTA & VisDrone & DeepFruits & MinneApple & ENA24 & iWildCam & Clipart & Comic & Watercolor & SKU110K & WIDER FACE & DeepFashion2 & iMaterialist & Kitchen & Oktoberfest & HollywoodHeads \cr \smidrulec
FRCN & COCO &
79.8 \scriptsize{$\pm$ 0.1} & 39.5 \scriptsize{$\pm$ 3.7} & 16.8 \scriptsize{$\pm$ 0.9} & 71.8 \scriptsize{$\pm$ 1.7} & 57.2 \scriptsize{$\pm$ 4.8} & 55.1 \scriptsize{$\pm$ 2.6} & \textbf{70.9} \scriptsize{$\pm$ 3.1} & \textbf{59.2} \scriptsize{$\pm$ 1.1} & 25.7 \scriptsize{$\pm$ 5.3} & 39.0 \scriptsize{$\pm$ 4.1} & 50.3 \scriptsize{$\pm$ 1.7} & 36.5 \scriptsize{$\pm$ 4.4} & 24.9 \scriptsize{$\pm$ 1.5} & 24.5 \scriptsize{$\pm$ 0.8} & 90.9 \scriptsize{$\pm$ 1.0} & 88.9 \scriptsize{$\pm$ 1.7} & \textbf{73.3} \scriptsize{$\pm$ 5.1} \cr
\rowcolor{Gray} & COCO &
80.2 \scriptsize{$\pm$ 0.4} & 41.7 \scriptsize{$\pm$ 3.5} & 18.0 \scriptsize{$\pm$ 0.9} & 72.8 \scriptsize{$\pm$ 1.6} & 58.5 \scriptsize{$\pm$ 5.0} & 55.9 \scriptsize{$\pm$ 2.5} & 68.7 \scriptsize{$\pm$ 3.0} & 53.2 \scriptsize{$\pm$ 0.7} & 22.2 \scriptsize{$\pm$ 4.2} & 34.7 \scriptsize{$\pm$ 3.7} & 49.9 \scriptsize{$\pm$ 2.0} & 37.8 \scriptsize{$\pm$ 2.6} & 27.1 \scriptsize{$\pm$ 1.6} & 25.4 \scriptsize{$\pm$ 0.9} & 93.0 \scriptsize{$\pm$ 0.9} & 91.7 \scriptsize{$\pm$ 1.8} & 68.9 \scriptsize{$\pm$ 4.8} \cr
\rowcolor{Gray} & FSODD &
79.3 \scriptsize{$\pm$ 0.5} & 38.8 \scriptsize{$\pm$ 3.7} & 14.1 \scriptsize{$\pm$ 0.6} & 75.0 \scriptsize{$\pm$ 2.2} & 56.9 \scriptsize{$\pm$ 3.3} & 59.3 \scriptsize{$\pm$ 3.0} & 67.6 \scriptsize{$\pm$ 3.4} & 35.9 \scriptsize{$\pm$ 1.3} & 16.7 \scriptsize{$\pm$ 2.2} & 26.8 \scriptsize{$\pm$ 2.8} & 46.5 \scriptsize{$\pm$ 2.0} & 31.0 \scriptsize{$\pm$ 3.1} & 29.1 \scriptsize{$\pm$ 1.2} & 24.5 \scriptsize{$\pm$ 0.9} & 90.3 \scriptsize{$\pm$ 1.1} & 91.3 \scriptsize{$\pm$ 1.7} & 67.7 \scriptsize{$\pm$ 3.0} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{80.6} \scriptsize{$\pm$ 0.5} & \textbf{44.0} \scriptsize{$\pm$ 3.8} & \textbf{19.6} \scriptsize{$\pm$ 0.8} & \textbf{76.8} \scriptsize{$\pm$ 1.8} & \textbf{60.4} \scriptsize{$\pm$ 5.3} & \textbf{62.6} \scriptsize{$\pm$ 3.1} & 70.2 \scriptsize{$\pm$ 2.9} & 58.6 \scriptsize{$\pm$ 0.9} & \textbf{28.8} \scriptsize{$\pm$ 4.9} & \textbf{41.6} \scriptsize{$\pm$ 4.2} & \textbf{52.3} \scriptsize{$\pm$ 1.4} & \textbf{42.2} \scriptsize{$\pm$ 2.7} & \textbf{31.3} \scriptsize{$\pm$ 1.5} & \textbf{29.7} \scriptsize{$\pm$ 1.0} & \textbf{93.3} \scriptsize{$\pm$ 0.6} & \textbf{93.2} \scriptsize{$\pm$ 1.7} & 72.8 \scriptsize{$\pm$ 3.9} \cr
\bottomrule
\multicolumn{2}{c}{10-shot} & \multicolumn{2}{c}{Logo} & \multicolumn{2}{c}{Medical} & \multicolumn{2}{c}{Person} & \multicolumn{2}{c}{Security} & Table & Text & \multicolumn{4}{c}{Traffic} & Underwater & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidruleb
Arch & Pre-train & LogoDet-3K & OpenLogo & ChestX-Det10 & DeepLesion & CrowdHuman & WiderPerson & PIDray & SIXray & table-detection & COCO-Text & Cityscapes & KITTI & LISA & TT100K & DUO \cr \smidrulec
FRCN & COCO &
60.0 \scriptsize{$\pm$ 5.1} & 27.7 \scriptsize{$\pm$ 2.0} & 10.9 \scriptsize{$\pm$ 0.7} & 2.1 \scriptsize{$\pm$ 0.9} & 52.0 \scriptsize{$\pm$ 1.4} & 57.2 \scriptsize{$\pm$ 1.8} & 35.1 \scriptsize{$\pm$ 3.4} & 35.2 \scriptsize{$\pm$ 2.2} & 53.5 \scriptsize{$\pm$ 11.1} & 10.6 \scriptsize{$\pm$ 1.5} & 42.0 \scriptsize{$\pm$ 3.1} & 49.8 \scriptsize{$\pm$ 2.6} & 57.8 \scriptsize{$\pm$ 4.2} & 25.9 \scriptsize{$\pm$ 4.1} & 40.6 \scriptsize{$\pm$ 3.0} & 45.8 \scriptsize{$\pm$ 2.1} & 3.0 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} & COCO &
65.4 \scriptsize{$\pm$ 3.4} & 30.8 \scriptsize{$\pm$ 2.4} & 12.5 \scriptsize{$\pm$ 0.9} & 2.1 \scriptsize{$\pm$ 0.8} & 54.4 \scriptsize{$\pm$ 1.5} & \textbf{60.0} \scriptsize{$\pm$ 1.0} & 37.7 \scriptsize{$\pm$ 2.6} & 35.8 \scriptsize{$\pm$ 2.3} & \textbf{54.0} \scriptsize{$\pm$ 8.2} & 13.5 \scriptsize{$\pm$ 2.2} & 42.1 \scriptsize{$\pm$ 2.6} & 52.0 \scriptsize{$\pm$ 2.8} & 63.9 \scriptsize{$\pm$ 5.0} & 26.3 \scriptsize{$\pm$ 3.8} & 44.3 \scriptsize{$\pm$ 2.4} & 46.7 \scriptsize{$\pm$ 1.6} & 2.4 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} & FSODD &
66.5 \scriptsize{$\pm$ 3.4} & 30.6 \scriptsize{$\pm$ 2.4} & 11.6 \scriptsize{$\pm$ 1.1} & 1.8 \scriptsize{$\pm$ 0.8} & 42.9 \scriptsize{$\pm$ 1.8} & 47.0 \scriptsize{$\pm$ 1.4} & 36.4 \scriptsize{$\pm$ 3.4} & 34.0 \scriptsize{$\pm$ 1.5} & 48.3 \scriptsize{$\pm$ 9.8} & 11.9 \scriptsize{$\pm$ 1.8} & 27.4 \scriptsize{$\pm$ 1.8} & 39.3 \scriptsize{$\pm$ 2.4} & 57.6 \scriptsize{$\pm$ 4.5} & 22.9 \scriptsize{$\pm$ 4.2} & 43.2 \scriptsize{$\pm$ 2.1} & 42.9 \scriptsize{$\pm$ 1.7} & 3.4 \scriptsize{$\pm$ 0.3} \cr
\rowcolor{Gray} \multirowcell{-3}{CRCN} & UniDet &
\textbf{69.7} \scriptsize{$\pm$ 3.7} & \textbf{37.1} \scriptsize{$\pm$ 2.2} & \textbf{13.1} \scriptsize{$\pm$ 0.9} & \textbf{3.0} \scriptsize{$\pm$ 1.1} & \textbf{55.6} \scriptsize{$\pm$ 1.5} & 59.8 \scriptsize{$\pm$ 1.2} & \textbf{43.3} \scriptsize{$\pm$ 3.5} & \textbf{40.0} \scriptsize{$\pm$ 2.3} & 53.2 \scriptsize{$\pm$ 9.9} & \textbf{16.1} \scriptsize{$\pm$ 2.4} & \textbf{46.1} \scriptsize{$\pm$ 2.9} & \textbf{53.6} \scriptsize{$\pm$ 3.2} & \textbf{65.6} \scriptsize{$\pm$ 5.1} & \textbf{30.3} \scriptsize{$\pm$ 4.5} & \textbf{46.9} \scriptsize{$\pm$ 2.2} & \textbf{49.7} \scriptsize{$\pm$ 1.9} & \textbf{1.2} \scriptsize{$\pm$ 0.3} \cr
\bottomrule
\end{tabular}
}
\caption{Performance of FT on all 32 datasets in the proposed benchmark with different model architectures and pre-training datasets.
%
FRCN stands for Faster R-CNN, CRCN stands for Cascade R-CNN.}
\label{tb:result_arch_32}
\end{sidewaystable*}


==> table_lvis_plus_cascade.tex <==
\begin{table*}[t]
\captionsetup{}
\def\smidrule{\cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}}
\def\smidrulf{\cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}\cmidrule(rl){6-6}}
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}[t]{cccccc}
\toprule
Arch & Pre-training & 1-shot & 3-shot & 5-shot & 10-shot  \cr \smidrulf
Cascade-RCNN-P67 & ImageNet &
13.5 \scriptsize{$\pm$ 1.6} & 23.2 \scriptsize{$\pm$ 1.5} & 29.5 \scriptsize{$\pm$ 1.2} & 37.7 \scriptsize{$\pm$ 1.2}  \cr
\rowcolor{Gray} Cascade-RCNN-P67 & COCO &
\textbf{35.4} \scriptsize{$\pm$ 1.8} & 44.7 \scriptsize{$\pm$ 1.6} & 49.9 \scriptsize{$\pm$ 1.2} & 56.4 \scriptsize{$\pm$ 1.1}  \cr
Cascade-RCNN-P67 & FSODD &
26.7 \scriptsize{$\pm$ 2.9} & 36.9 \scriptsize{$\pm$ 1.5} & 42.3 \scriptsize{$\pm$ 1.2} & 49.1 \scriptsize{$\pm$ 1.0}  \cr
\rowcolor{Gray} Cascade-RCNN-P67 & LVIS &
34.4 \scriptsize{$\pm$ 2.0} & 44.0 \scriptsize{$\pm$ 1.6} & 48.7 \scriptsize{$\pm$ 1.4} & 55.6 \scriptsize{$\pm$ 1.0}  \cr
Cascade-RCNN-P67 & Unified &
33.3 \scriptsize{$\pm$ 2.2} & 44.3 \scriptsize{$\pm$ 1.4} & 49.6 \scriptsize{$\pm$ 1.2} & 56.6 \scriptsize{$\pm$ 1.1}  \cr
Cascade-RCNN-P67 & LVIS+ &
34.7 \scriptsize{$\pm$ 4.2} & \textbf{46.6} \scriptsize{$\pm$ 1.6} & \textbf{52.0} \scriptsize{$\pm$ 1.0} & \textbf{59.0} \scriptsize{$\pm$ 1.0}  \cr
\hline
\hline
\rowcolor{Gray} CenterNet2 & COCO &
29.1 \scriptsize{$\pm$ 5.2} & 40.2 \scriptsize{$\pm$ 1.9} & 45.3 \scriptsize{$\pm$ 1.8} & 52.5 \scriptsize{$\pm$ 1.9}  \cr
CenterNet2 & LVIS &
28.1 \scriptsize{$\pm$ 3.3} & 39.0 \scriptsize{$\pm$ 1.7} & 44.3 \scriptsize{$\pm$ 1.2} & 51.6 \scriptsize{$\pm$ 1.0}  \cr
\rowcolor{Gray} CenterNet2 & LVIS+ &
34.9 \scriptsize{$\pm$ 3.2} & 46.5 \scriptsize{$\pm$ 1.9} & 51.8 \scriptsize{$\pm$ 1.3} & 58.8 \scriptsize{$\pm$ 1.0}  \cr
CenterNet2 & LVIS++ &
\textbf{35.8} \scriptsize{$\pm$ 3.4} & \textbf{47.2} \scriptsize{$\pm$ 2.1} & \textbf{52.6} \scriptsize{$\pm$ 1.4} & \textbf{59.4} \scriptsize{$\pm$ 1.1}  \cr
\bottomrule
\end{tabular}
}
\caption{The effect of pre-training dataset with Cascade-RCNN-P67 and CenterNet2.}
\label{tab:pre_training_overall_en}
\end{table*}
\vspace{-3pt}


==> table_tune.tex <==
\begin{table*}[t]
\def\smidruleb{\cmidrule(rl){1-1}\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}\cmidrule(rl){6-6}\cmidrule(rl){7-7}\cmidrule(rl){8-8}\cmidrule(rl){9-9}\cmidrule(rl){10-10}\cmidrule(rl){11-11}\cmidrule(rl){12-12}\cmidrule(rl){13-13}}
\def\smidrulea{\cmidrule(rl){2-2}\cmidrule(rl){3-3}\cmidrule(rl){4-4}\cmidrule(rl){5-5}\cmidrule(rl){6-6}\cmidrule(rl){7-7}\cmidrule(rl){8-8}\cmidrule(rl){9-9}\cmidrule(rl){10-10}\cmidrule(rl){11-11}}
%
\centering
\caption{The effect of tuning more parameters.}
\label{tb:result_5-shot}
%
\begin{subtable}[h]{\textwidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
\multirowcell{2}{5-shot} & Aerial & Agriculture & Animal & Cartoon & Fashion & Food & Logo & Person & Security & Traffic & \multirowcell{2}{Mean} & \multirowcell{2}{Rank} \cr \smidrulea
 & VisDrone & DeepFruits & iWildCam & Clipart & iMaterialist & Oktoberfest & LogoDet-3K & CrowdHuman & SIXray & KITTI \cr \smidruleb
%
Tuning FC layer (TFA-fc~\cite{wang2020frustratingly}) & 10.1 \scriptsize{$\pm$ 0.6} & 47.5 \scriptsize{$\pm$ 1.8} & \textbf{71.7} \scriptsize{$\pm$ 2.4} & 40.2 \scriptsize{$\pm$ 2.6} & 8.0 \scriptsize{$\pm$ 0.9} & 41.1 \scriptsize{$\pm$ 4.8} & 14.2 \scriptsize{$\pm$ 3.7} & 30.6 \scriptsize{$\pm$ 0.8} & 7.9 \scriptsize{$\pm$ 2.0} & \textbf{48.3} \scriptsize{$\pm$ 3.4} & 32.0 \scriptsize{$\pm$ 1.3} & 2.7 \scriptsize{$\pm$ 0.2} \cr
\rowcolor{Gray} Tuning Detection Head (FSCE-base~\cite{sun2021fsce}) & 13.0 \scriptsize{$\pm$ 0.7} & 59.2 \scriptsize{$\pm$ 3.2} & 70.6 \scriptsize{$\pm$ 1.7} & 43.5 \scriptsize{$\pm$ 2.5} & 20.5 \scriptsize{$\pm$ 0.9} & 70.7 \scriptsize{$\pm$ 3.5} & 47.2 \scriptsize{$\pm$ 3.5} &\textbf{51.6} \scriptsize{$\pm$ 2.0} & 15.9 \scriptsize{$\pm$ 2.2} & 47.1 \scriptsize{$\pm$ 4.3} & 43.9 \scriptsize{$\pm$ 1.1} & 1.9 \scriptsize{$\pm$ 0.2} \cr
Tuning Whole Network (FT) & \textbf{14.2} \scriptsize{$\pm$ 0.8} & \textbf{60.7} \scriptsize{$\pm$ 3.8} & 63.3 \scriptsize{$\pm$ 5.7} & \textbf{49.3} \scriptsize{$\pm$ 3.5} & \textbf{21.3} \scriptsize{$\pm$ 0.8} & \textbf{81.6} \scriptsize{$\pm$ 4.0} & \textbf{49.8} \scriptsize{$\pm$ 3.5} & 51.5 \scriptsize{$\pm$ 2.2} & \textbf{23.9} \scriptsize{$\pm$ 3.9} & 45.3 \scriptsize{$\pm$ 3.7} & \textbf{46.1} \scriptsize{$\pm$ 1.4} & \textbf{1.5} \scriptsize{$\pm$ 0.2} \cr
\bottomrule
\end{tabular}
}
\label{tab:tune}
\end{subtable}
%
\end{table*}

